Language-Embedded Gaussian Splats (LEGS): Incrementally Building Room-Scale Representations with a Mobile Robot

Building semantic 3D maps is valuable for searching for objects of interest in offices, warehouses, stores, and homes. We present a mapping system that incrementally builds a Language-Embedded Gaussian Splat (LEGS): a detailed 3D scene representation that encodes both appearance and semantics in a unified representation. LEGS is trained online as a robot traverses its environment to enable localization of open-vocabulary object queries. We evaluate LEGS on 4 room-scale scenes where we query for objects in the scene to assess how LEGS can capture semantic meaning. We compare LEGS to LERF and find that while both systems have comparable object query success rates, LEGS trains over 3.5x faster than LERF. Results suggest that a multi-camera setup and incremental bundle adjustment can boost visual reconstruction quality in constrained robot trajectories, and suggest LEGS can localize open-vocabulary and long-tail object queries with up to 66% accuracy.

==> acks.tex <==
\section*{Acknowledgement}
This research was performed at the AUTOLAB at UC Berkeley in affiliation with the Berkeley AI Research (BAIR) Lab. The authors were supported in part by donations from  Bosch, Toyota Research Institute, Google, Siemens, and Autodesk and by equipment grants from PhotoNeo, NVidia, and Intuitive Surgical. The research is also supported by C3.ai Digital Transformation Institute for AI resilience. 


==> chapters/concurrent_work.tex <==
\section{Concurrent work}



 

==> tables/cost.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}
        {@{}l | @{\quad}c@{\quad} | c@{\quad}  | c@{\;} c@{\quad}c@{\;}c@{\;}c@{}}\toprule
                    & Server &Single &  \multicolumn{3}{c}\algname  \\
         Application & Core      &Server &   On-Demand  & & {Spot VM} \\ \midrule
         YOLO & 16  & 0.40 (1.17x) &    0.80 (2.34x)     & & {0.34 (1x)}   \\ % spot 0.17
         SAM & 4$^*$  & 0.53 (1.21x) &    1.06 (2.42x)    & & {0.44 (1x)} \\ % spot 0.223
         % MPT-Apartment & 16   &0.90 (1.09x)  &  1.80 (2.18x)  &{0.82 (1x)} &  \\ % spot 0.17
         MPT-Home        & 32   &1.79 (1.05x) & 3.58 (2.10x)  & &{1.69 (1x)} \\ 
         MPT-Cubicles & 32  &1.79 (1.05x) &   3.58 (2.10x)    & &{1.69 (1x) }  \\ 
         MPT-TwistyCool & 64 &3.58 (2.13x) &  7.16 (4.26x)  & &{1.68 (1x)}  \\ 
        Pick-Scan-Place & 16  & 0.40 (1.17x) &    0.80 (2.34x)     & & {0.34 (1x)}    \\ 
         \bottomrule
    \end{tabular}
    \caption{\textbf{\algname hourly cost saving comparison to a Single-Server (one on-demand machine)} \algname can use two on-demand machines deployment or spot VMs. In SAM, we use Nvidia T4 GPU accelerator for the inference. \algname is cheaper to run 2 spot VMs as opposed to a single server deployment up to 2.13x. \jeff{unclear, is this table showing USD/hour?  If so, label it in the column headers.} \jeff{Switch to booktabs, see latex comment for URL} } % https://nhigham.com/2019/11/19/better-latex-tables-with-booktabs/
    \label{tab:eval:cost}
\end{table}


% \begin{table}[t]
%     \centering
%     \footnotesize
%     \begin{tabular}
%         {@{}l | @{\quad}c@{\quad} | c@{\quad} c@{\;} c@{\quad}c@{\;}c@{\;}c@{}}\toprule
%           & Hardware & \multicolumn{3}{c}{Cost (US\$ per Hr)} \\
%           & Used &   Single-Server & \algname \\ \midrule
         
%          % Dex-Net & T4 GPU & 0.53 (1.21x) & 1.04 (2.36x) & 0.44 \\ % spot 0.223

%          \bottomrule
%     \end{tabular}
%     \caption{\textbf{\algname hourly cost saving compared to a Single-Server (one on-demand machine) and Fault Tolerant (FT) (two on-demand machines) deployment on Vision-based Cloud Robotics} \eric{I tend to remove this table: I think the benefit of fault tolerance is clear, and we don't show as much benefit in terms of cost. I think we can do a "one more thing" later in the physical experiment section. }  }
%     \label{tab:eval:cost}
% \end{table}


==> tables/exp1results.tex <==
% \begin{table}
%     \centering
%     \footnotesize
%     \begin{tabular}{l l l r r } 
% \toprule
%  & Available & Failure  & Prob. Selecting  & Failure \\ 
% & Machines  & Rate (\%)& Edge(\%) &  Reduction\\
% \midrule
% 1&E-M, E-B    & 26.67 (8/30) & - & 1x, \textbf{2.2x} \\
% 2&E-M, C-W    & 6.67 (2/30)     & 30 (9/30)   &  \textbf{4x}, 1.3x \\
% 3&E-B, C-W     & 10.00 (3/30)    &  6.67 (2/30) & \textbf{5.6x}, 1x\\ 
% 4&E-M, C-E      & 30.00 (9/30)  & 46.67 (14/30) & 1x, \textbf{1.1x} \\ 
% 5&E-B, C-E      & 53.33  (16/30)   &  3.33 (1/30)  &  \textbf{1.1x}, 0.63x \\ 
% 6&E-M, C-W, C-E       &  10.00 (3/30)  & 53.33 (16/30) & 2.7x, 1x, \textbf{3.3x} \\  
% 7&E-B, C-W, C-E       &  6.67 (2/30)  & 0 (0/30)  & \textbf{8.5x}, 1.5x, 5x \\  
% \bottomrule
% \end{tabular}
% \caption{\textbf{Evaluation of \algname in Failure Reduction} \algname selects from available baseline machines and we measure the failure rate (lower the better). \algname matches or surpasses the performance of the best individual machine, reducing the failure rate by up to 8.5 times. By selecting a machine with best latency at a given moment, it can achieve even lower failure rate than up to 1.5 times lower than that of any single machine available. \eric{please help check with the numbers, i did the calculation by hand}}
% \label{tab:eval:exp1:results}
% \vspace{-8pt}
% \end{table}

% \begin{table}
%     \centering
%     \footnotesize
%     \begin{tabular}{l l l l } 
% \toprule
%  Failure & Delay: 20 + 50ms   &  Delay: 20 + 50ms\\ 
%  Rate(\%) & 50\%   Applied     &  100\%  Applied  \\
% \midrule
% Edge1(Delay) &  26.7(8/30)  &  56.7 (17/30)        \\
%     + Edge 2 &  0.0  &  0.0       \\
%     + Cloud(West) &  10.0(3/30)  &  6.7   \\
%     + Cloud(East) &  30.0(9/30)  &  53.3   \\
%     + Cloud(East) + Cloud(West) &  6.7(2/30)   &  10.0   \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Evaluation of \algname in Failure Reduction} \algname selects from available baseline machines and we measure the failure rate (lower the better). \algname matches or surpasses the performance of the best individual machine, reducing the failure rate by up to 8.5 times. By selecting a machine with best latency at a given moment, it can achieve even lower failure rate than up to 1.5 times lower than that of any single machine available.}
% \label{tab:eval:exp1:results}
% \vspace{-8pt}
% \end{table}

\begin{table*}
    \centering
    \setlength{\tabcolsep}{10pt} 
    \renewcommand{\arraystretch}{1.5} % Default value: 1

    \footnotesize
    \begin{tabular}  {l | c | c c c c c c} 
\toprule
 % Failure Rate & Edge 1(Delay)  &  Edge 1(Delay) & Edge 1(Delay) & Edge 1(Delay) \\ 

 Edge 1 (Add Delay) & Edge 1 & Edge 1 & & & \\ 
 Failure Rate (\%)  & Only & + Edge 2     &  + Cloud(W) & + Cloud(E) & + Cloud(W) + Cloud(E)  \\
\hline
 100\% Applied &  56.7\% & 0.0\% & 10.0\% & 30.0\% & \bf{6.7\%}    \\
 % \midrule
    (Failure Reduction) &   & $(\infty)$ & (5.7x) & (1.9x) & \bf{(8.5x)}    \\
\hline
    50\% Applied &  26.7\%  & 0.0\% & \bf{6.7\%} & 53.3\% & 10.0\%  \\
% \midrule
   (Failure Reduction) &   &  ($\infty$) & \bf{(4.0x)} & (0.5x) & (2.7x)  \\
    % + Cloud(East) + Cloud(West) &  6.7(2/30)   &  10.0   \\
\bottomrule
\end{tabular}

\caption{\textbf{When local network was congested, \algname reduced failures:} Upon application of random network delays on Edge \#1, \algname automatically re-route to alternative services, i.e. Edge 2, Cloud(W), Cloud(E).  
Such automatic switching functionality to an alternative, location independent service(s) improves robustness of the system and reduced failure rate (lower the better) of the overall system. 
\algname matches performance of the best individual machine, reducing the failure rate by up to 8.5 times by selecting the best available machine compared to single edge service system under heavy network congestion.
We also showed that \algname enabled flexible yet reliable access to open cloud services via Anycast to reduce failure rate.}
\label{tab:eval:exp1:results}
\vspace{-8pt}
\end{table*}

==> tables/exp1setup.tex <==
\begin{table}
    \centering
    \footnotesize
    \begin{tabular}{ l l l | c c } 
\toprule
 & Candidates & Failure  & Interference  & Interference\\ 
  &          & Rate (\%)& (ms) & Prob. (\%)\\
\midrule
 E-G&Edge (Good)    & 0 (0/30)     & 0     & 0\\
 E-M&Edge (Medium)  & 26.67 (8/30) & $35\pm15$ & 50\\ 
 E-B&Edge (Bad)     & 56.67 (17/30)  & $35\pm15$ & 100\\ 
 C-W&Cloud (West US)     & 10  (3/30)   & -     & -\\ 
 C-E&Cloud (East US)       &  36.67 (10/30)  & -     & -\\ 
\bottomrule
\end{tabular}
\caption{\textbf{Failure Rate and Network Setups of Baseline Machines For Visual Distance Estimation}  The robot controller maintains a direct and stable connection to the Edge server via an Ethernet cable. Interference is introduced with a $35\pm15$ ms network delay, applied at rates of 50\% and 100\% to respectively represent Edge (Medium) and Edge (Bad) conditions. All the robots and edge servers are at California (West US), and the Cloud servers are located at AWS facilities in Oregon (West US) and Ohio (East US). \eric{is 35+-15 the same as 20 + 50? the latter one might be confusing} \marcus{Michael says it's just $50 \pm 0$ ms (no randomness).}
}
\label{tab:eval:exp1:setup}
\vspace{-8pt}
\end{table}

==> tables/time.tex <==

% column: application, experiment time, average uptime, total preemptions 
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{@{}l@{\quad}c@{\quad} c@{\quad}c@{\quad}c@{\quad}c@{\;}c@{\;}c@{}}\toprule
           & Experiment & Preemptions & 1 Response  & 2 Response &  \\
           &  Time (hr) & Experienced & Rate (\%)  & Rate (\%)  \\
         \midrule
        
         YOLO &  25  & 2 & 100 & 75  \\
         SAM  &  25  & 3  & 100  & 75 \\ 
         Dex-Net  &  25  &  3 & 100  & 75 \\ 
         MPT  &  25  & 3  & 100  &75 \\ 
         \bottomrule
    \end{tabular}
    \caption{\textbf{\algname experiment uptime on Cloud Robotics applications} We run all cloud robotics applications with more than 24 hours period and experienced more than 2 preemptions. \algname is able to provide at least one response for all the applications despite the preemptions, and with X \% of receiving responses from multiple servers.\eric{response rate are placeholders}  }
    \label{tab:eval:time}
\end{table}

